Tackling Corruption With Agents & ICT: A Vision

Corruption is universally considered as an undesirable characteristic of public services. But despite attempts to simplify and automate such services, there is very little prior work to detect, handle or prevent corruption in computation literature. This is particularly surprising given the significant advances made in detecting fraud, a relevant but different form of public impropriety afflicting businesses. In this paper, we paint a vision of how information and communications technology (ICT), and specifically agent-based methods, can help tackle corruption in public services and identify challenges to achieve the vision.

==> automation.tex <==

% ------------------------------------------------------------------
% ------------------------------------------------------------------

\section{Process Automation and Corruption}
\label{sec:automation}

In this section, we investigate explore why automating public processes helps
tackle corruption and to what extent. We follow the automation approach recommended 
in \cite{autoseek} and, using the $\Aniti$ meta-model, discuss where automation helps
in tackling corruption.

%We first give a background of different issues 
%that one needs to consider before automating parts of a process.
%Then we propose a modest  approach for automation from literature \cite{autoseek} 
%by mapping the types of activities in a process to the suggested type of automation 
%policies that can be used for them without significant effort on writing or validating them. 
%Finally we articulate using the corruption meta-model how automation helps.

% ------------------------------------------------------------------
\subsection{Characterizing the Activities at a Process Step}


 % -------------------- 
   \begin{figure}
   \centerline{
   \epsfxsize=180pt
   \rotatebox{0}{\epsfbox{fig/step-processing.eps}}}
   \caption{{\em Information Processing Occurring at a Process Step (above) and when
                it is automated (below).}}
   \label{fig:step-proc}
   \end{figure}
 % -------------------- 
 


%A service delivery process consists of steps describing activities. 
%Figure~\ref{fig:step-proc} shows what happens in a process step.
As shown in Figure~\ref{fig:step-proc}, an activity (or task) step consumes information about input, does processing and produces output. The information about output records that the process has taken place. The types of processing occurring at a step can be classified as:
\begin{enumerate}
\item Checking of information (I-type): Here, the activity involves checking 
      correctness of input,
      testing its validity, entitlement or applicability.  
\item	Making simple decisions and acting (S-type). Here, the activity is to check data 
      value that 
      leads to statically enumerable set of decisions (e.g., if a personnel is unassigned,
      then it can be applied to a proposed task).
\item Making complex decisions and acting (C-type). Here, the activity is to  check data values 
      and apply the knowledge of sub-system behavior collectively to make decisions 
      (e.g., if rice is facing shortage, whether wheat can be a reasonable sustitute for procurement).
\end{enumerate}

 
%Now, before automating a step, one needs to figure out the desirable role of a person performing the task. Do we want generalists or specialist? In most automation strategies, 
%the human performers are seen as specialists who are focused on making (complex) decisions which uses the knowledge about the services sub-system much more effectively. The information check and simple decisions are distractions to them and are ideal candidates for automation. 
%
%
%% ------------------------------------------------------------------
%\subsection{The Spectrum of Automation Choices}

 

To automate any process, control inputs are additionally needed to let the process 
step know what behavior is expected. A correct automated process will use the control 
and input information, and produce the same output information as that produced by a non-automated process. Control information are:
%\begin{enumerate}
%\item	
(1) {\bf Condition}: which is a state that is being checked at that step. The automated agent, 
      who knows what to do in the condition, will simply check the condition
      and execute the activity accordingly.
%\item 
(2) {\bf Prescriptive policies}:
      which are important conditions to monitor and the actions to 
      take in those conditions\cite{eca}. The agent uses control information to 
			act accordingly based on the prevailing state.
%\item	
(3) {\bf Declarative policies}: are goal that are desired from the step for a particular set of 
      inputs\cite{weld-aimag}. The agent needs to find the course of actions that achieves 
      the goals and execute them.
%\item	
(4) {\bf Utility policies}: are utilities of what goals are important to achieve in different   
      conditions\cite{utility-ac}. The agent has to select the goals of the specific condition
      based on utility, decide about the course of actions that will achieve the
      goals, and execute them.
%\end{enumerate}


%There are many standard choices based on the complexity of providing 
%control information and verifying whether the automated system worked correctly.
%The Event-Condition-Action (ECA) rules\cite{eca} are an example of prescriptive 
%policies. The area of planning in AI\cite{weld-aimag} deals with how to 
%generate a course of actions to achieve goals. They
%can handle both declarative as well as utility-based policies\cite{utility-ac}. An 
%example of a system which
%can support many types of policies is ABLE\cite{able-planning}. 

In the Autoseek methodology\cite{autoseek}, the automation approach is to do cost-benefit analysis of 
a step process to 
%\begin{enumerate}
%\item	
(a) fully automate information checking steps through conditions,
%\item	
(b) simplify and partially automate simple decision making steps through 
      prescriptive policies, and
%\item	
(c) focus the human agents to complex decisions and explore declarative and
      utility policies over time. 
%\end{enumerate}



% ------------------------------------------------------------------

\subsection{How Automation Helps Tackle Corruption}
\label{sec:auto-help}

When a process is automated, the access to its inputs is made readily available for the computer programs
to execute. Further, the old (I-type) steps are eliminated thus leading to both improved data
access and quality. If automation is moderate, the criteria in (S-type) steps of the process are  enumerated. Doing so removes discretion from the (S-type) steps even if only a few of the steps
may be actually automated. If (C-type) steps are also automated, provided they are cost-effective from implementation point-of-view, the process will provide consistently similar output to all requests thereby making corruption detection, as defined in this paper, impossible. 

In practice, just doing (I-type) automation and enumerating criteria for (S-type) decision goes a long way in bringing transparency to the process and removing discretion.


% ------------------------------------------------------------------
% ------------------------------------------------------------------


==> discussion.tex <==

% -------------------------------------------------------------------
% -------------------------------------------------------------------
\section{Open Data and Corruption}

%\comment{Nidhi/ Biplav: to add}

Open data\cite{od} is a well entrenched idea in science that data should be
available to everyone. In the government space, the idea of opening up data, 
coupled with using it using semantic assertions, called {\em linked data} \cite{ld-book}, 
is favorably viewed for economic growth\cite{od-impact}. For example, a study
has noted that EU Open Government Data policies can
boost direct business activity by up to €40 billion per year
(0.3\% of EU's GDP), and the overall benefit, including
direct and indirect effects, could be up to €200 billion per
year (1.7\% of GDP). 

Open Data can also be helpful to tackle corruption\cite{corruption-opendata}. Suppose
statistics about each service request for public services is collected, anonymized and 
then published to general public. The information may cover request details like
type of request and requester demographics, and the outcome including whether it 
was succesfully completed, the time and 
cost incurred by both the requester and the provider. This data, when analyzed in
aggregate, and in correlation with the established SLAs covering time and cost, can provide
unprecedented visibility. 
 %This is because
%it provides visibility about what services were completed and with what 
%SLAs (time and cost). 
The increased transparency drives accountability and reduces the economic loss
due to corruption. 

% -------------------------------------------------------------------
% -------------------------------------------------------------------



==> evaluation.tex <==

% -------------------------------------------------------------------
% -------------------------------------------------------------------



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation by Illustration}
\label{sec:demo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We evaluate our framework by applying it to two case studies from the
public services domain - international driving permit (Figure~\ref{fig:idp}) and
national registration (Figure~\ref{fig:id}).  Here, 
rectangular boxes refer to {\em activities}, diamond boxes are {\em decisions} and greyed boxes refer to {\em inputs} or {\em outputs}. All activities shown are manual.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{International Driving Permit (IDP)}
\label{sec:idp}

In the IDP example (Figure~\ref{fig:idp}), there is service {\em execution cost} specified (of Rs 500) but no service {\em execution time} given.  There is no 
{\em escalation} mechanism. In the context of corruptibility patterns, we note that:


\begin{itemize}
\item  The decision node, {\em Are the documents valid?}, is discretionary because
    it is subjective with no clear mechanism to check it. In contrast, the check   
		whether all documents have been submitted is objective.
\item  For a service request, the process does not have time bound SLAs although 
    it does have cost-based SLA.  
\item The IDP is monopolistic since only a single authority (RTO) can process it.
\item The process  has little reviewability and low visibility since there is no escalation mechanism.
    
\end{itemize}

Now consider the IDP in USA\cite{aaa}. The procedure involves filling a form online, visiting
the office of an authorized agency with a valid state-issued driver's license, photos and 
fees, and getting the permit. Here, there are multiple agencies to process the request and the 
prerequisite driver license can be verified objectively (e.g., with social security databases). 

Compared with IDP in India, there is no monopoly and less discretion.
The process can be further improved from corruption standpoint by defining service level limits on processing time, providing an escalation mechanism and publishing statistics about requests completed.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{National Registration}
\label{sec:eval-id}


In the ID example (Figure~\ref{fig:id}), there is neither service {\em execution cost} specified 
nor service {\em execution time} are specified.  There is no 
{\em escalation} mechanism. In the context of corruptibility patterns, we note that:


\begin{itemize}
\item  The decision node, {\em 3 - vetting}, and the activity, {\em 13 - verify identity}, are discretionary with no clear mechanism on how to accomplish them. 
  In contrast, the checks for documents having been submitted are objective.
\item  There is no SLA for the process.  
\item The ID process is monopolistic since only a single authority (registration office) can process it.
\item The process  has little reviewability and low visibility since there is no escalation mechanism.
    
\end{itemize}

Now consider the national registration processes in USA, called social security (SS) \cite{ssn-us},
and in India, called Aadhar \cite{aadhar-india}. In SS,  a clear list of documents proving
US citizenship (or legal residence), age and identity is listed. There is little room for discretion
because no category allows a signed attestation by a high-level official to be acceptable - something
allowed in Kenya. The cost and time limits for the service are prescribed. The process, however, can only be handled by a single agency creating a monopoly.

In the case of Aadhar in India \cite{aadhar-india}, 18 Proofs of Identity (PoI) and   33 Proofs of Address (PoA) documents are permitted for making the request. The process also allows discretion
by allowing attested documents from high-level officials. The cost and time limits for the service are prescribed. The process, however, can only be handled by a single agency creating a
monopoly.


Thus, the proposed model allows us to compare the national registration processes of three countries
from corruption perspective. We observe that the Kenyan process is more corruptible than the Indian 
Aadhar process, which in turn is more corruptible that the USA' SS process.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







% -------------------------------------------------------------------
% -------------------------------------------------------------------



==> relatedwork.tex <==

% -------------------------------------------------------------------
% -------------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:literature}


%\comment{Nirmit/Biplav: Fin all relevant works and differentiate.}
%
%\subsection{Related Work}
%Apart from those discussed earlier, we now relate  our work to major work.
The known mechanisms for detecting corruption are  a) survey based, where public opinion surveys is used to measure the perceived corruption or b) institutional diagnostics such as audits and 
anti-corruption policy conformance of a public institution\cite{corr-tools}. 
The drawback of survey is that they are subjective and prone to human bias while
institutional diagnostics only assess the administrative loop holes and do not take care of scenarios where beneficiaries collude in corrupt practices. Moreover both mechanisms are reactive and not
preventive.
%The drawback of survey based methods is that they are subjective and prone to human bias. On the other hand institutional diagnostics only assess the administrative loop holes and do not take care of scenarios where beneficiaries collude in corrupt practices. Moreover both these mechanism are reactive rather than preventive.

The importance of a formal model has long been felt but the lone example we are aware of
is \cite{corruption-credit-formalmodel} which presents a model to connect informal and formal
credit markets.
In business process community, there is work on patterns and anti-patterns for capturing
desirable service attributes\cite{patterns}. However, this has not been applied for 
detecting corruption
in public services.

% -------------------------------------------------------------------
% -------------------------------------------------------------------


